Reducing the Teacher-Student Gap via Spherical Knowledge Disitllation

Knowledge distillation aims at obtaining a compact and effective model by learning the mapping function from a much larger one. Due to the limited capacity of the student, the student would underfit the teacher. Therefore, student performance would unexpectedly drop when distilling from an oversized teacher, termed the capacity gap problem. We investigate this problem by study the gap of confidence between teacher and student. We find that the magnitude of confidence is not necessary for knowledge distillation and could harm the student performance if the student are forced to learn confidence. We propose Spherical Knowledge Distillation to eliminate this gap explicitly, which eases the underfitting problem. We find this novel knowledge representation can improve compact models with much larger teachers and is robust to temperature. We conducted experiments on both CIFAR100 and ImageNet, and achieve significant improvement. Specifically, we train ResNet18 to 73.0 accuracy, which is a substantial improvement over previous SOTA and is on par with resnet34 almost twice the student size. The implementation has been shared at https://github.com/forjiuzhou/Spherical-Knowledge-Distillation.

==> 0_intro_zh.tex <==
Hinton指出，许多昆虫由两个阶段，在幼虫阶段的形态，有利于从环境中摄取能量和营养。而另一个形态适合飞行和繁殖。例如，当毛毛虫变成蝴蝶后，原来有利于摄取营养的觅食系统，在成虫阶段就被抛弃。而其中的营养和能量保留了下来。
这个比喻是十分有效的，它启发我们，应该在训练和部署时采用不同的模型。训练时采用较大的模型，然后将知识蒸馏到一个小模型上用于部署。自那以后，知识蒸馏方法就流行了起来。

然而，这一方法有他的问题。
然而，在实践中，蒸馏方法却遭遇了capacity gap问题。
对capacity gap的描述。

幼虫变为成虫后，幼虫复杂的消化系统不再被成虫所需要，相反会伤害到成虫的生存。同样的，teacher中也会存在一些不利于学生的因素。我们期待小模型能够在拟合大模型的输出中获得性能提升，
然而，这一拟合可能会遇到一些困难，作为训练目标的teacher的输出，可能包含了一些不利于学生泛化的归纳偏好。
% 然而，teacher的输出中可能包含了一些学生难以拟合的归纳偏好。
在训练teacher时，为了将数据集的知识编码到模型中，通常会采用最大化对ground truth预测的负对数概率值的做法。
secondary information
然而，这一做法却同时会让模型倾向于对被预测的类别赋予较高的概率值，从而形成一个比较sharp的概率分布。
而小模型在拟合这个sharp的模型时，面临了困难，因此导致了capacity gap。
% 就模型泛化而言，我们需要的不是对被预测类别赋予尽可能大的概率值，而是当面对新模型时，学生能够给出正确的预测，那么学生需要学习teacher的这一sharp的特性吗？

图例，logits->概率
越大的模型越自信，最终目标是one-hot。
学生难以拟合

由于模型的softness，是由logits的norm控制的。我们可以使用norm衡量模型的softness。我们通过实验证明，example 的norm并不包含可以让学生提升性能的信息，相反，由于难以拟合，会伤害学生的性能，在很大程度上组成了capacity gap。


我们提出了skd
怎么怎么样
与拟合norm不同，skd使用固定的norm，从而专注于学习teacher输出中真正有用部分的知识。
温度

4.0 蒸馏是什么样的
4.1.0 capacity gap是什么样的
    loss
    acc
4.1.1 对capacity gap的分析
4.1.2 不同配置的teacher变化时，norm loss的变化
4.1.3 两个实验

5.0 skd
5.1 skd对于capacity gap
5.2 skd对于temperature


6. exp
cifar100
imagenet
模型事实上不需要学习各个样本的norm，而只需要一个足够撑起表示空间的norm

7. discussion 
需要考虑模型本身的归纳偏好，来定义合适的知识。
% 大模型相比小模型，会倾向于形成尖锐的概率分布，而这个性质，事实上是不包含知识的。
训练目标要考虑模型的归纳偏好。
从teacher的角度看，知识反映了数据集中的一些特征。但是从学生的角度看，知识作为训练目标，需要考虑学生的归纳偏好。

能不能说这个归纳偏好不是知识？恐怕不能？更像是难以拟合的部分
只能说这个归纳偏好难以拟合，难以让学生提升性能。

abs
如果将模型看成是一个映射，一个大模型的输出，可以
知识蒸馏考虑如何将知识、
从teacher的角度看，知识反映了数据集中的一些特征。但是从学生的角度看，知识作为训练目标，需要考虑学生的归纳偏好。
忽略了学生和教师模型本身的归纳偏好是不同的。正是因为欠缺了这个考虑，导致了capacity gap。我们做了什么，怎么样解决了这个问题。效果如何


知识蒸馏通过train a model by a well-trained larger model to get a 小而美得模型。the method follows such intuition that a larger model can better capture some ``dark knowledge'', which highly reflected in its generalization, ...
Thus how to represent knowledge, or what should be tranfered between models, is critical for KD. As the pioneer in KD, hinton ..... Following this work, other researchers proposed a lot of variation .....
But the problem, named capacity gap, always confuses this field. According to the assumaption of KD, larger teacher -> better performance. 但事实不是这样，大的teacher带不来提升，甚至下降~（引用hinton）。有人专门解决这样问题，..... 这里我们提出一种新的知识表征方式来解决这样问题，我们希望 为了实现此目标，我们研究了哪些因素会导致（原始）KD取得成功，以及哪些因素会伤害学生的性能。
我们发现norm既不是泛化信息，也不是可转移的。而方向才反映了泛化性，而且也更易于转移。

我们提出了一种球形知识表示形式来满足以上两个目的。
球形知识是怎么做的，为什么解决了以上问题。

还发现参数更为鲁棒。
